Efficient Agents: Building Effective Agents While Reducing Cost

The remarkable capabilities of Large Language Model (LLM)-driven agents have enabled sophisticated systems to tackle complex, multi-step tasks, but their escalating costs threaten scalability and accessibility. This work presents the first systematic study of the efficiency-effectiveness trade-off in modern agent systems, addressing the critical need for cost-effective designs without sacrificing performance. We investigate three key questions: (1) How much complexity do agentic tasks inherently require? (2) When do additional modules yield diminishing returns? (3) How much efficiency can be gained through the design of efficient agent frameworks? Through an empirical analysis on the GAIA benchmark, we evaluate the impact of LLM backbone selection, agent framework designs, and test-time scaling strategies. Using the cost-of-pass metric, we quantify the efficiency-performance trade-off across these dimensions. Our findings inform the development of Efficient Agents , a novel agent framework that has an optimal complexity to task requirements. Efficient Agents retains 96.7% of the performance of OWL, one leading open-source agent framework, while reducing operational costs from $0.398 to $0.228, resulting in a 28.4% improvement in cost-of-pass. Our work provides actionable insights for designing efficient, high-performing agent systems, advancing the accessibility and sustainability of AI-driven solutions.

==> src/Limitations.tex <==
\section*{Limitations}
Despite our efficient agent significantly reducing the cost for intelligent agent systems to solve complex problems, our study has three key limitations: our method was exclusively implemented and evaluated within the SmolAgents framework, making its generalizability to other general agent frameworks unverified; its efficiency across other task types is currently unknown; and we only explored initial, fixed agent configurations, lacking dynamic efficiency optimization during problem-solving.

==> tables/reflection.tex <==
\begin{table*}[h]
\centering
\caption{The impact of Reflection module on effectiveness and efficiency.}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|cccc|cccc|cccc|cccc}
\toprule
& \multicolumn{4}{c|}{Efficiency} & \multicolumn{4}{c|}{Effectiveness} & \multicolumn{8}{c}{Cost} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-17}
& \multicolumn{4}{c|}{cost-of-pass$\downarrow$} & \multicolumn{4}{c|}{Acc.$\uparrow$} & \multicolumn{4}{c|}{Cost/\textdollar$\downarrow$} & \multicolumn{4}{c}{\#Tokens$\downarrow$} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
Reflection & all & l1 & l2 & l3 & all & l1 & l2 & l3 & all & l1 & l2 & l3 & all & l1 & l2 & l3 \\
\midrule
w/o & 0.98 & 0.32 & 1.07 & 3.51 & 53.33 & 69.81 & 50.00 & 30.77 & 0.521 & 0.227 & 0.533 & 1.080 & 242K & 102K & 249K & 506K \\
w/ & 1.15 & 0.60 & 1.09 & 3.72 & 56.97 & 69.81 & 55.81 & 34.62 & 0.653129 & 0.419 & 0.610 & 1.286 & 492K & 326K & 474K & 897K \\

\bottomrule
\end{tabular}
}
\label{tab:reflection}
\end{table*}

